Digital Twin as a Service (DTaaS): A Platform for Digital Twin Developers and Users

Establishing digital twins is a non-trivial endeavour especially when users face significant challenges in creating them from scratch. Ready availability of reusable models, data and tool assets, can help with creation and use of digital twins. A number of digital twin frameworks exist to facilitate creation and use of digital twins. In this paper we propose a digital twin framework to author digital twin assets, create digital twins from reusable assets and make the digital twins available as a service to other users. The proposed framework automates the management of reusable assets, storage, provision of compute infrastructure, communication and monitoring tasks. The users operate at the level of digital twins and delegate rest of the work to the digital twin as a service framework.

==> sections/dt-lifecycle-old.tex <==

\begin{figure*}
	\centering
	\begin{subfigure}{0.35\textwidth}
		\includegraphics[width=1.0\textwidth]{images/dt-components}
		\caption{Constitution of a minimum viable DT. At least one asset from mandatory set is required. An executable binary asset is a valid DT.}
		\label{fig:assets}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.35\textwidth}
		\includegraphics[width=1.0\textwidth]{images/dt-composability}
		\caption{Composability among DTs. Composition introduces recursion in the construction of DTs.}
		\label{fig:composability}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.25\textwidth}
		\includegraphics[width=1.1\textwidth]{images/dt-config}
		\caption{Configuration possibilities for DTs. Flat configuration is more flexible yet more complex.}
		\label{fig:config}
	\end{subfigure}
	
	\caption{Data, Model, Function, Tool, ready to use Digital Twin assets of the DT platform. The DT configuration links assets to form a meaningful DT.}
	\label{fig:dt-properties}
\end{figure*}





\section{Digital Twin Lifecycle} \label{sec:dtlife}

\subsection{DT Assets}\label{sec:dt-assets}

The DTaaS software platform treats DTs as having reusable assets. These assets are put together and configured in a certain way. We use four categories of assets: data (D), model (M), function (F) and Tool (T).

The data (D) asset refers to data sources and sinks available to a DT. Typical examples of data sources are sensor measurements from the PT, and test data provided by manufacturers for calibration of models. Typical examples of data sinks are visualization software, external users and data storage services. There exist special outputs such as events, and commands which are akin to control outputs from a DT. These control outputs usually go to the PT, but they can also go to another DT~\cite{Esterle2021}.

The model (M) assets are used to describe different aspects of a PT and its environment, at different levels of abstraction. Therefore, it's possible to have multiple models for the same PT. For example, a flexible robot used in a car production plant may have structural model(s) which will be useful in tracking the wear and tear of parts. The same robot can have a behavioral model(s) describing the safety guarantees provided by the robot manufacturer. The same robot can also have a functional model(s) describing the part manufacturing capabilities of the robot.

The function (F) assets are primarily responsible for pre and post-processing of: data inputs, data outputs, control outputs. The research results from data science can be used to create useful function assets for the platform.
In some cases, DT models require calibration prior to their use; functions written by domain experts along with right data inputs can make model calibration an achievable goal. Another use of functions is to process the sensor and actuator data of both the PT and the DT.


The software tool (T) assets are software used to create, evaluate and analyze models. These tools are executed on top of a computing platforms, i.e., an operating system, or virtual machines like Java virtual machine, or docker containers. The tools tend to be platform specific, making them less reusable than models. 
A tool can be packaged to run on a local or distributed virtual machine environments thus allowing selection of most suitable execution environment for a DT. 
Most models require tools to evaluate them in the context of data inputs. 
There exist cases where executable packages are run as binaries in a computing environment. Each of these packages are a pre-packaged combination of models and tools put together to create a ready to use DT.

There is a dependency between the assets especially in the context of creating DTs. These dependencies are illustrated in Figure~\ref{fig:assets}. 
Only functions/tools can use models/data. 
A specific combination of these assets constitute a DT. The interconnections between assets, parameters (configurable run-time variables) of the assets need to be specified for each DT. This information becomes a part of the DT asset configuration ($C_{c}$). The information encoded in $C_c$ is not sufficient to truly manifest a closed loop communication between DT and PT. Let $C_{dt}$ be this complete configuration for the DT.

The possibilities of asset combinations used in a DT can be expressed using Equation~\ref{eq:dt-def}. 
A PT like a factory consists of multiple robots each of which can be have a DT of their own. This hierarchical aggregation is to replicate the compositional properties of a PT. A hierarchical DT can also use the elementary DT assets in addition to the aggregated DTs \cite{Esterle2021}. Figure~\ref{fig:composability} shows this possibility.

\begin{comment}
\begin{align}\label{eq:dt-regex}
	D_t: & D{^*}M^{*}(FT)^{+}C_{dt} \\
	& (DMFT)^{*}D^{+}_{t}C_{dt}\notag	
\end{align}
\end{comment}

\vspace*{-12pt}
\begin{align}\label{eq:dt-def}
	D_t: & \{ D{^*},M^{*},(FT)^{+} \}C_{dt} \\
	& \{ (DMFT)^{*},D^{+}_{t} \}C_{dt}\notag	
\end{align}

where D denotes data, M denotes models, F denotes functions, T denotes tools, $C_{dt}$ denotes DT configuration and $D_t$ is a symbolic notation for a DT itself. The Equation~\ref{eq:dt-def} shows two possible mathematical representations for a DT created from reusable assets. The  $\{ D{^*},M^{*},(FT)^{+} \}C_{dt}$ expression denotes composition of DT from D,M,T and F assets. The $\{ (\mathit{DMFT})^{*},D^{+}_{t} \}C_{dt}$ expression represents use of one DT and other reusable assets to create another DT.

\begin{comment}
\begin{table*}
	\renewcommand{\arraystretch}{1.3}
	\caption{Different possible regex combinations and their use in the application domains. Each combination provides different utility for the users of DTs.}
	\label{tab:dt-config}
	\centering
	\begin{tabular}{p{1in}p{2in}p{3in}}
		\toprule
		\bfseries Components in a DT & \bfseries DT Utility & \bfseries Use cases\\
		\midrule
		$[FT]^+C_{dt}$ & generators (for scenario analysis) & 
			\vspace*{-12pt}
			\begin{enumerate}
				\item factory output due to unstable raw material supplies
				\item test double for physical twin
			\end{enumerate}
		\\
		
		$\{D^{+},[FT]^+\}C_{dt}$ & events, faults, extract-transform-load (ETL) & 
			\vspace*{-12pt}
			\begin{enumerate}
				\item Thermal runaway in a furnace
				\item graphical view of a city as seen by sensors
			\end{enumerate}
		\\
		
		\{$D^{*},[FT]^{+},M^{+}\}C_{dt}$ & component analysis & 
			\vspace*{-12pt}
			\begin{enumerate}
				\item gas flow in a pipe
				\item deformation analysis on a bridge
			\end{enumerate}
			\\
		
		$\{[DFMT]^{*},D^{+}_{t}\}C_{dt}$ & hierarchical DTs & 
		\vspace*{-12pt}
		\begin{enumerate}
			\item city DT using DTs of suburbs and airport
			\item plant DT using DTs of robots
		\end{enumerate}
		\\

		\bottomrule
	\end{tabular}
\end{table*}
\vspace{12pt}
Some meaningful DT compositions, their potential benefits and example use cases are shown in Table~\ref{tab:dt-config} \cg{dangling ref}. Complex applications may demand different insights from DTs. Thus the chosen DT assets must be amenable to change in response to changing environments.
\end{comment}


\subsection{DT Configuration}
\cg{we may have to tell the reader that we abstain from trying to define these configurations more concretely, because that is outside the scope of the this paper.}
The DT asset configuration ($C_{c}$ introduced in Section~\ref{sec:dt-assets}) is only a part of the complete configuration needed for running a live DT with feedback loop to the PT. The $C_{pt}$ denotes configuration information required by DT to communicate with PT. Each DT may have constraints on the kind of execution environments it is capable of using, i.e. tools that can only run either on a specific operating system or on a server with specific hardware capabilities. The $C_i$ denote the infrastructure configuration required by a DT. The $C_e$ denote configuration for integration of a DT with external software systems, ex. third-party visual dashboards.
%In addition, a DT requires information about its' PT and the configuration for communication protocols to be used for bidirectional communication with its PT; let $C_{pt}$ denote this configuration. Each DT may have constraints on the kind of execution environments it is capable of using, for example tools that can only run either on a specific operating system or on a server with specific hardware capabilities; let $C_i$ denote the infrastructure configuration. In addition, often times users require integration of DTs with external software systems, ex. with third-party visual dashboards; let $C_e$ denote this configuration. 
In the case of hierarchical DTs, there may be a need to provide configuration ($C_{dt}$) for each of the DTs included. Equation~\ref{eq:dt-config} defines DT config for a hierarchical DT. In case of non-hierarchical DTs, $l = 0$ and $C^{l}_{dt} = \phi$. 
Figure~\ref{fig:config} shows a graphical illustration of the relationship between $C_{dt}$ and all other configurations. A sanity check is required on validity of any given $C_{dt}$.  \phm{eq2: can a hierarchical dt only consist of one dt?}

\begin{equation}\label{eq:dt-config}
	C^{l+1}_{dt} = \{ C_c, C_i, C_e, C_{pt},C^{l}_{dt} \}
\end{equation}
% Can we say something about the DSL for DT configuration??

Two situations demand adjustments to $C_{dt}$. One is a user-driven change in any of $C_{c}$, $C_{pt}$, $C_i$, $C_e$, or $C_{dt}$ of included DTs. In this case, a validity check is required before a transition to new a configuration can be made. Second is a requirement to perform what-if analysis. 
What-if analysis requires minor variations on $C_{dt}$ to plan and optimize future steps to be undertaken either on a PT or a DT. 
\cg{Do we really wish to keep the variations stored in the DT as new configurations? I would expect only some of these variations (optimal ones in come sense), to be recorded. And note that it's variations of the assets of the DT, which ok maybe lead to variations in the DT but we could make that more explicit. Is that what we mean in the prev sentence?}
Actual implementation of what-if analysis can be resource intensive with the resource requirements scaling up in proportion to algorithmic bounds on the (sub)-systems being used by a DT.

A DT can also use external tools such as planning and optimization. This is especially true in what-if analysis. If these tools are used exclusively within a DT, then they can be considered as tools in asset library. Otherwise, they are part of the infrastructure / external world.


\subsection{Phases in DT Lifecycle}
\label{sec:dt_phases}

A DT lifecycle consists of create, execute, persist, analyze, evolve and terminate phases. In addition to having D,M,T and F as assets in the library, the ready to use DTs can also be a library assets. 
Users might choose to create a new DT or select an existing DT. The create phase involves asset selection and an specifying DT configuration.  
If DT is reused, there is no creation phase at the time of reuse. 
The execute phase involves automated execution of a DT based on its configuration. 
If a DT is reused, there will be a temporal gap between creation and execution times of a DT. Thus, a need might arise for just-in-time DT reconfiguration at the point of execution. \prasad{one sentence on analyze phase}. The evolve phase involves user/event-triggered reconfiguration of an instantiated DT. The persist phase involves saving the state of DT to enable future recovery. The terminate phase involves stopping the execution of DT and releasing all the resources and connections mentioned in the DT configuration.


\paragraph*{Reconfiguration and Consistency}
The evolution phases require to reconfigure DTs. The aim of reconfiguration is to ensure \emph{consistency} between the DT and PT,  i.e., the adequacy of the DT to mirror the PT, access its data, and enable the required analyses. 


Reconfigurations may be triggered by different kinds of events, two of which we discussed above, they are specific to the system and, thus, reconfiguration procedures must be provided by the user. These procedures are highly application specific, but reuse the application agnostic services. The reconfiguration procedures must be able to access the current DT configuration and its assets. As the configuration is highly heterogenous, the platform should offer a way for \emph{uniform} access to it, i.e., a representation mapping $\mu$ that is defined on $C_{dt}$ \emph{and all its assets} as well as provide an interface for the user to program reconfigurations in terms of the uniform access, i.e., define transitions
$\mu\left(C^{l}_{dt}\right) \rightarrow_\mu \mu\left(C^{l+1}_{dt}\right).$


Knowledge graphs are a suitable technology to implement for the mappings. Knowledge graphs that has been established 
to express structures and unify data access~\cite{HoganBCdMGKGNNN21}, and for which numerous mappings, mature tools and techniques exist.
In particular, mappings for software~\cite{KamburjanKSJG21} and approaches to express consistency between (mapped) DT and PT (through a top-down asset model~\cite{bickford_operationalizing_2020}) 
in terms of queries on knowledge graphs have been investigated~\cite{KamburjanJ22}. 

\prasad{Please rephrase the text from here to the end of the section in terms of analyze and/or evolve DT lifecycle phases. There is only one sentence explaining all of Figure \ref{fig:dt-overview-slide}? Is it possible to remove it and cite \cite{Feng2021}? \cg{Done, but I'm still confused. The MAPE-K loop evolves models, not digital twins. MAybe we need to have a call? One possible interpretation of what you want is that you want an example of the analyze and evolve stages, in terms of the incubator. If that's the case, then I can help, but until I'm certain, it's better not to waste time. Also, I may have commented out the wrong figure... maybe you referred to the wrong figure in your request.}}
Monitoring, at its most basic level, requires data gathering and storage, of the interaction between the PT and its environment, and among the PT's assets.
However, even for a simple system such as an incubator (like the one introduced in \cite{Feng2021}), monitoring requires that hidden quantities (that is, quantities for which we cannot obtain a sensor measurement directly) be estimated.
\cg{Prasad, pls check:}This activity corresponds to the \textbf{analyze} lifecycle stage.
Often these hidden quantities are represented by variables in the various models used by the DT.
The consequence is that estimates of these hidden quantities need to be stored in the database, becoming then input to decision-making simulations, where all variables of the models need to be properly initialized. 
%This is why Fig \ref{fig:dt-overview-slide} shows data flowing from the monitors to the decision making processes.
For more details we refer the reader to \cite{Feng2021a}.

% \begin{figure}[htb]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{images/dt-overview-slide}
% 	\caption{asassa.}
% 	\label{fig:dt-overview-slide}
% \end{figure}

Monitoring also informs the next lifecycle stage of the DT: the \textbf{evolve} stage.
Consider one example through the MAPE-K loop introduced in \cite{Arcaini2015} and instantiated for a simple incubator system in \cref{fig:MAPEK_Loop}, and suppose the lid of the incubator is openned. The execution of the loop is summarized in the figure.
Note that the monitoring and planning steps make use of the other DT services.

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.45\textwidth]{images/MAPEK_Loop}
	\caption{MAPE-K loop. Adapted from \cite{Feng2022a}. Note the links between the MAPE-K stages and the DT lifecycle introduced in \cref{sec:dt_phases}.}
	\label{fig:MAPEK_Loop}
\end{figure}

% \cg{Input on the importance of environment in the calibration of DT}
% Note that the performance on the calibration process has a direct impact in the subsequent steps of the PT reconfiguration. \prasad{This is the first time PT reconfiguration is being mentioned. Perhaps a bit more explanation will help?} Consider Fig \ref{fig:MAPEK_Loop}, and imagine that not enough data was gathered after the anomaly is detected, so that the calibration was inaccurate. 
% The consequence is that the control policy is likely to be sub-optimal, which may, in turn, cause more reconfigurations in the future.
% Also note the trade-off between gathering enough data for a successful calibration, moving fast enough to the control policy optimization, and reconfiguring the PT.
% Taking more time in any of these stages will likely yield better results, at the cost of higher delay in reconfiguring the system.


\subsection{Hierarchical DTs (Composition of DTs)}
\label{sec:dt?composition}

\cg{Revisit each of the points: how do they change:}
\begin{itemize}
	\item DT Assets
	\item DT Configuration
	\item DT Lifecicle
\end{itemize}


==> sections/usecase.tex <==
\section{Incubator Use Case}
\begin{tcolorbox}
	\begin{enumerate}
		\item Text describing the incubator physical twin (Hao)
		\item Incubator digital twin description (Hao)
		\item DT config and execution (Prasad)
		\item results interpretation (Hao)
	\end{enumerate}
\end{tcolorbox}


\begin{figure*}
	\centerline{\includegraphics[scale=0.15]{images/incubator-results}}
	\caption{Synchronization and remote control of incubator physical twin from the digital twin.}
	\label{fig:incubator-graph}
\end{figure*}






